On the Expressive Power of the Normal Form for Branching-Time Temporal Logics

With the emerging applications that involve complex distributed systems branching-time specifications are specifically important as they reflect dynamic and non-deterministic nature of such applications. We describe the expressive power of a simple yet powerful branching-time specification framework -- branching-time normal form (BNF), which has been developed as part of clausal resolution for branching-time temporal logics. We show the encoding of Buchi Tree Automata in the language of the normal form, thus representing, syntactically, tree automata in a high-level way. Thus we can treat BNF as a normal form for the latter. These results enable us (1) to translate given problem specifications into the normal form and apply as a verification method a deductive reasoning technique -- the clausal temporal resolution; (2) to apply one of the core components of the resolution method -- the loop searching to extract, syntactically, hidden invariants in a wide range of complex temporal specifications.

==> eptcsdata.tex <==
\providecommand{\firstpage}{254}
\providecommand{\publicationstatus}{A. Indrzejczak, M. Zawidzki (Eds): 10th International Conference\\on Non-Classical Logics. Theory and Applications (NCL 2022)\\
EPTCS 358, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.358.19}{10.4204/EPTCS.358.19}}

